A survey of symbolic methods for establishing equivalence-based properties in cryptographic protocols

Cryptographic protocols aim at securing communications over insecure networks such as the Internet, where dishonest users may listen to communications and interfere with them. A secure communication has a different meaning depending on the underlying application. It ranges from the confidentiality of a data to e.g. verifiability in electronic voting systems. Another example of a security notion is privacy. Formal symbolic models have proved their usefulness for analysing the security of protocols. Until quite recently, most results focused on trace properties like confidentiality or authentication. There are however several security properties, which cannot be defined (or cannot be naturally defined) as trace properties and require a notion of behavioural equivalence. Typical examples are anonymity, and privacy related properties. During the last decade, several results and verification tools have been developed to analyse equivalence-based security properties. We propose here a synthesis of decidability and undecidability results for equivalence-based security properties. Moreover, we give an overview of existing verification tools that may be used to verify equivalence-based security properties.

==> refs.tex <==
@article{CCD-tocl15,
   author = {Chr{\'e}tien, R{\'e}my and Cortier, V{\'e}ronique and Delaune, St{\'e}phanie}, 
   OPTDOI = {10.1145/2811262}, 
   journal = {ACM Transactions on Computational Logic}, 
   month = sep, 
   number = {1:3}, 
   publisher = {ACM Press}, 
   title = {From security protocols to pushdown automata}, 
   OPTurl = {http://www.lsv.ens-cachan.fr/Publis/PAPERS/PDF/CCD-tocl15.pdf}, 
   volume = {17},
   year = {2015}, 
}



@InProceedings{MiSa92,
  author = 	 {Milner, R. and Sangiorgi, D.},
  title = 	 {Barbed Bisimulation},
  OPTcrossref =  {},
  OPTkey = 	 {},
  booktitle = {Proc.\ 19th International Colloquium on Automata, Languages, and
                   Programming ({ICALP}'92)},
  year = 	 {1992},
  editor = 	 {Kuich, W.},
  volume = 	 {623},
  OPTnumber = 	 {},
  series = 	 {LNCS},
  pages = 	 {685--695},
  OPTmonth = 	 {},
  OPTaddress = 	 {},
  OPTorganization = {},
  publisher = {Springer Verlag},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@article{ThayerHG99-jcs,
  author    = {F. Javier Thayer and
               Jonathan C. Herzog and
               Joshua D. Guttman},
  title     = {Strand Spaces: Proving Security Protocols Correct},
  journal   = {Journal of Computer Security},
  volume    = {7},
  number    = {1},
  pages     = {191--230},
  year      = {1999},
  OPTurl       = {http://content.iospress.com/articles/journal-of-computer-security/jcs117},
  }

@inproceedings{CervesatoDLMS99,
  author    = {I. Cervesato and
               N. Durgin and
               P. Lincoln and
               J. Mitchell and
               A. Scedrov},
  title     = {A Meta-Notation for Protocol Analysis},
  booktitle = {Proc.\  12th Computer Security Foundations Workshop ({CSFW}'99)},
  year      = {1999},
  pages     = {55-69},
  publisher =     {IEEE Computer Society Press},
  OPTaddress   =   {Mordano (Italy)}, 
  
}


@inproceedings{Geraud-outil,
  author    = {P. Henry and
               G. S{\'e}nizergues},
  title     = {LALBLC A Program Testing the Equivalence of dpda's},
  year      = {2013},
  pages     = {169-180},
  booktitle     = {Proc.\ 18th International
               Conference on Implementation and Application of Automata ({CIAA}'13)},
address = {Halifax, NS, Canada},
  publisher = {Springer},
  series    = {LNCS},
  volume    = {7982},
}

@inproceedings{DRS-ifiptm08,
   author = {Delaune, St{\'e}phanie and Ryan, Mark D. and Smyth, Ben}, 
   booktitle = {{P}roc.\  2nd {J}oint i{T}rust and {PST} {C}onferences on {P}rivacy, {T}rust {M}anagement and {S}ecurity (IFIPTM'08)}, 
   pages = {263-278}, 
   publisher = {Springer}, 
   series = {IFIP Conference Proc.\ }, 
   title = {Automatic verification of privacy properties in the applied pi-calculus}, 
   volume = {263}, 
   year = {2008}, 
}


@inproceedings{CCD-concur14,
   author = {Chr{\'e}tien, R{\'e}my and Cortier, V{\'e}ronique and Delaune, St{\'e}phanie}, 
   booktitle = {{P}roc.\  25th {I}nternational {C}onference on {C}oncurrency {T}heory ({CONCUR}'14)}, 
   pages = {372-386}, 
   publisher = {Springer}, 
   series = {LNCS},
   title = {Typing messages for free in security protocols: the~case of equivalence properties}, 
   volume = {8704}, 
   year = {2014}, 
}

@inproceedings{CCD-csf15,
   author = {Chr{\'e}tien, R{\'e}my and Cortier, V{\'e}ronique and Delaune, St{\'e}phanie}, 
   booktitle = {{P}roc.\  28th {C}omputer {S}ecurity {F}oundations {S}ymposium ({CSF}'15)}, 
   pages = {170-184}, 
   publisher = {{IEEE} Computer Society Press}, 
   title = {Decidability of trace equivalence for protocols with nonces}, 
   year = {2015}, 
}


@inproceedings{rta03,
  author =        {H. Comon-Lundh and V. Cortier},
  booktitle =     {14th Proc.\ International Conference on Rewriting Techniques
                   and Applications ({RTA}'2003)},
  pages =         {148-164},
  publisher =     {Springer},
  series =        {LNCS},
  title =         {New Decidability Results for Fragments of First-Order
                   Logic and Application to Cryptographic Protocols},
  volume =        {2706},
  year =          {2003},
}

@Article{CCCK16,
  author =	 {Chadha, Rohit and Cheval, Vincent and
                  Ciob{\^a}c{\u{a}}, {\c{S}}tefan and Kremer,
                  Steve},
  title =	 {Automated verification of equivalence properties of
                  cryptographic protocol},
  journal =	 {ACM Transactions on Computational Logic},
  year =	 2016,
  url =		 {https://hal.inria.fr/hal-01306561/document},
  note =         {To appear}
}


@inproceedings{DKP-ijcar12,
   author = {Delaune, St{\'e}phanie and Kremer, Steve and Pasail{\u{a}}, Daniel}, 
   booktitle = {{P}roc.\ 6th {I}nternational {J}oint {C}onference on {A}utomated {R}easoning ({IJCAR}'12)}, 
   pages = {164-178}, 
   publisher = {Springer-Verlag}, 
   series = {LNAI},
   title = {Security protocols, constraint systems, and group theories}, 
   volume = {7364}, 
   year = {2012}, 
}


@article{chevalier10,
  author = 	 {Yannick Chevalier and Michael Rusinowitch},
  title = 	 {Decidability of Symbolic Equivalence of Derivations},
  journal = 	 {Journal of Automated Reasoning},
   volume    = {48},
  number    = {2},
  pages     = {263--292},
  year      = {2012}
}


@article{DSV03,
  author    = {Luca Durante and
               Riccardo Sisto and
               Adriano Valenzano},
  title     = {Automatic testing equivalence verification of spi calculus
               specifications},
  journal   = {ACM Transactions on Software Engineering and Methodology},
  volume    = {12},
  number    = {2},
  year      = {2003},
  pages     = {222-284},
}



@ARTICLE{BorealeNicolaPuglieseJoC02,
  AUTHOR = {M.Boreale and R. De Nicola and R. Pugliese},
  TITLE = {Proof Techniques for Cryptographic Processes},
  JOURNAL = {SIAM Journal on Computing},
  YEAR = 2002,
  VOLUME = 31,
  NUMBER = 3,
  PAGES = {947--986}
}



@inproceedings{DKR-csfw06,
   author = {Delaune, St{\'e}phanie and Kremer, Steve and Ryan, Mark D.}, 
   booktitle = {{P}roc. 19th  {C}omputer {S}ecurity {F}oundations {W}orkshop ({CSFW}'06)}, 
   pages = {28-39}, 
   publisher = {{IEEE} Computer Society Press}, 
   title = {Coercion-Resistance and Receipt-Freeness in Electronic Voting}, 
   year = {2006}, 
}

@article{AbadiGordon99,
  author    = {Mart\'{\i}n Abadi and
               Andrew D. Gordon},
  title     = {A Calculus for Cryptographic Protocols: The spi Calculus},
  journal   = {Information and  Computation},
  volume    = {148},
  number    = {1},
  year      = {1999},
  pages     = {1-70},
}



@inproceedings{AC04Icalp,
  author =        {M. Abadi and V. Cortier},
  booktitle =     {Proc.\  31st International Colloquium on Automata, Languages, and
                   Programming ({ICALP}'04)},
  title =         {Deciding Knowledge in Security Protocols under
                   Equational Theories},
  year =          {2004},
  publisher =     {Springer-Verlag},
  series     =    {LNCS},
  volume =        {3142},
  pages =         {46-58},
}


@InProceedings{AC05,
  author =       {Abadi, M. and V. Cortier},
  title =        {Deciding knowledge in security protocols under (many more) equational theories},
  booktitle =    {Proc.\ 18th Computer Security Foundations Workshop (CSFW'05)},
  year =         {2005},
  publisher =    {IEEE Computer Society Press},
  pages     =    {62-76},
}

@inproceedings{dolev81security,
  author =    {D. Dolev and  A. C. Yao},
  title =     {On the Security of Public Key Protocols},
  booktitle = {Proc.  22nd  Symposium on Foundations of Computer Science ({FCS}'81)},
  publisher = {IEEE Computer Society Press},
  pages =     {350-357},
  year =      {1981},
}


@inproceedings{UC-unruh13,
  author    = {Florian B{\"{o}}hl and
               Dominique Unruh},
  title     = {Symbolic Universal Composability},
  booktitle = {Proc.\ 26th Computer Security Foundations Symposium ({CSF}'13)},
  pages     = {257--271},
  year      = {2013},
  publisher = {{IEEE} Computer Society Press},
}


@InProceedings{CanettiFOCS01,
  author =       {Ran Canetti},
  title =        {Universally Composable Security: A New Paradigm for Cryptographic Protocols},
  booktitle = {Proc.\ 42nd Annual Symposium on Foundations of Computer Science ({FOCS}'01)},
  pages =        {136-145},
  year =         {2001},
  OPTaddress =      {Las Vegas (Nevada, USA)},
  publisher = {IEEE Computer Society Press},
}


@inproceedings{DKP-fsttcs09,
   author = {Delaune, St{\'e}phanie and Kremer, Steve and Pereira, Olivier}, 
   booktitle = {{P}roc.\ 29th {C}onference on {F}oundations of {S}oftware {T}echnology and {T}heoretical {C}omputer {S}cience ({FSTTCS}'09)}, 
   pages = {169-180}, 
   publisher = {Leibniz-Zentrum f{\"u}r Informatik}, 
   series = {Leibniz International Proc.\  in Informatics}, 
   title = {Simulation based security in the applied pi calculus}, 
   volume = {4}, 
   year = {2009}, 
}


@inproceedings{DJP-fast10,
  	author =	{Dong, Naipeng and Jonker, Hugo and Pang, Jun},
  	booktitle =	{{P}roceedings of the 7th {I}nternational {W}orkshop on {F}ormal {A}spects in {S}ecurity and {T}rust ({FAST}'10)},
     pages = {223-238},
        volume = {6561},
   publisher = {Springer},
        series = {LNCS},
	title =	{Analysis of a receipt-free auction protocol in the applied pi calculus},
  	year =	{2010}
}

@inproceedings{DLL-post13,
  author =	  {Dreier, Jannik and  Lafourcade, Pascal and  Lakhnech, Yassine},
  booktitle =     {{P}roc.\ 2nd {C}onferences on {P}rinciples of {S}ecurity and {T}rust (POST'13)},
  publisher =     {Springer},
  series =        {LNCS},
  title =         {Formal Verification of e-Auction Protocols},
  pages = {247-266},
volume =     {7796},
  year =          {2013},
  }



@inproceedings{ACKR-post13,
  author =	  {Arapinis, Myrto and Cortier, V{\'e}ronique and Kremer, Steve and Ryan, Mark D.},
  booktitle =     {{P}roc.\ 2nd {C}onference on {P}rinciples of {S}ecurity and {T}rust (POST'13)},
  OPTeditor =        {Basin, David and Mitchell, John},
  pages =         {21-40},
  publisher =     {Springer},
  series =        {LNCS},
  title =         {{P}ractical {E}verlasting {P}rivacy},
  volume =        {7796},
  year =          {2013},
  }

@inproceedings{BenalohT94,
  author    = {Josh Benaloh and Dwight Tuinstra},
  title     = {Receipt-free secret-ballot elections (extended abstract)},
  booktitle = {Proc.\  26th Symposium on Theory of Computing ({STOC}'94)},
  year      = {1994},
  pages     = {544-553},
  publisher = {ACM Press},
  OPTaddress   = {Montr{\'e}al, Qu{\'e}bec},
}


@inproceedings{BackesVote08,
  author    = {Michael Backes and
               Catalin Hritcu and
               Matteo Maffei},
  title     = {Automated Verification of Remote Electronic Voting Protocols
               in the Applied Pi-Calculus},
  year      = {2008},
  pages     = {195-209},
  booktitle     = {Proc.\  21st Computer Security Foundations
               Symposium, (CSF'08)},
  publisher = {IEEE Computer Society Press}
}



@InProceedings{lowe97hierarchy,
  author = 	 {G. Lowe},
  title = 	 {A Hierarchy of Authentication Specifications},
  booktitle = {Proc.\ 10th Computer Security Foundations Workshop (CSFW'97)},
  pages = 	 {18-30},
  year = 	 {1997},
  publisher = {IEEE Computer Society Press},
}

@inproceedings{KremerRyan2005,
  author =      {S. Kremer and M. D. Ryan},
  booktitle =   {Proc.\ 14th {E}uropean {S}ymposium on {P}rogramming ({ESOP}'05)},
  pages =       {186-200},
  publisher =   {Springer-Verlag},
  series =      {LNCS},
  title =       {Analysis of an Electronic Voting Protocol in the Applied Pi-Calculus},
  volume =      {3444},
  year =        {2005},
}

@article{DiffieHelman76,
  author =        {W. Diffie and M. Hellman},
  journal =       {Transactions on Information Society},
  number =        {6},
  pages =         {644-654},
  title =         {New Directions in Cryptography},
  volume =        {22},
  year =          {1976},
  publisher =     {IEEE Computer Society Press},
}

@article{RSA78,
  author    = {R. Rivest and
               A. Shamir and
               L. Adleman},
  title     = {A Method for Obtaining Digital Signatures and Public-Key
               Cryptosystems},
  journal   = {Communications of the ACM},
  volume    = {21},
  number    = {2},
  year      = {1978},
  pages     = {120-126},
}



@TechReport{ICAO-Passport,
  OPTauthor = 	 {{PKI} Task Force},
  title = 	 {{PKI} for machine readable travel documents offering {ICC} read-only access},
  institution =  {International Civil Aviation Organization},
  year = 	 {2004},
  OPTkey = 	 {},
  OPTtype = 	 {},
  OPTnumber = 	 {},
  OPTaddress = 	 {},
  OPTmonth = 	 {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}


@inproceedings{esop03,
  author =        {Comon{-}Lundh, Hubert and Cortier, V{\'e}ronique},
  booktitle =     {{P}roc.\  12th {E}uropean {S}ymposium on
                   {P}rogramming ({ESOP}'03)},
  pages =         {99-113},
  publisher =     {Springer},
  series =        {LNCS},
  title =         {Security properties: two agents are sufficient},
  volume =        {2618},
  year =          {2003},
}

@article{esop03journal,
  author =        {Comon{-}Lundh, Hubert and Cortier, V{\'e}ronique},
  journal =       {Science of Computer Programming},
  month =         mar,
  number =        {1-3},
  pages =         {51-71},
  publisher =     {Elsevier Science Publishers},
  title =         {Security Properties: {T}wo Agents are Sufficient},
  volume =        {50},
  year =          {2004},
}

@InProceedings{AbadiFournet2001,
  author =       {M. Abadi and C. Fournet},
  title =        {Mobile Values, New Names, and Secure Communication},
  booktitle =    {Proc.\ 28th  Symposium on Principles of
                  Programming Languages (POPL'01)},
  pages =        {104-115},
  year =         {2001},
  publisher =    {ACM Press},
}

@inproceedings{Fast-2011,
  author    = {Bruno Conchinha and
               David A. Basin and
               Carlos Caleiro},
  title     = {{FAST:} An Efficient Decision Procedure for Deduction and Static Equivalence},
  booktitle = {Proc.\ 22nd International Conference on Rewriting Techniques
               and Applications, ({RTA}'11)},
  pages     = {11--20},
  year      = {2011},
  series    = {LIPIcs},
  volume    = {10},
  publisher = {Schloss Dagstuhl - Leibniz-Zentrum fuer Informatik},
}



@article{CD-jar10,
   author = {Cortier, V{\'e}ronique and Delaune, St{\'e}phanie}, 
   journal = {Journal of Automated Reasoning}, 
   month = apr, 
   number = {4}, 
   pages = {441-487}, 
   publisher = {Springer}, 
   title = {Decidability and combination results for two notions of knowledge in security protocols}, 
   volume = {48}, 
   year = {2012}, 
}

@article{CDK-jar10,
   author = {Ciob{\^a}c{\u{a}}, {\c{S}}tefan and Delaune, St{\'e}phanie and Kremer, Steve}, 
   journal = {Journal of Automated Reasoning}, 
   month = feb, 
   number = {2}, 
   pages = {219-262}, 
   publisher = {Springer}, 
   title = {Computing knowledge in security protocols under convergent equational theories}, 
   volume = {48}, 
   year = {2012}, 
}

@article{BCD-tocl12,
   author = {Baudet, Mathieu and Cortier, V{\'e}ronique and Delaune, St{\'e}phanie}, 
   journal = {ACM Transactions on Computational Logic}, 
   month = feb, 
   number = {1:4}, 
   publisher = {ACM Press}, 
   title = {{YAPA}: A~generic tool for computing intruder knowledge},
   volume = {14}, 
   year = {2013}, 
}

@inproceedings{BDH-concur15,
  	author =	{Baelde, David and Delaune, St{\'e}phanie and Hirschi, Lucca},
  	booktitle =	{{P}roc.\ 26th {I}nternational {C}onference on {C}oncurrency {T}heory ({CONCUR}'15)},
  	pages =	{497-510},
  	publisher =	{Leibniz-Zentrum f{\"u}r Informatik},
  	series =	{LIPIcs},
	title =	{Partial Order Reduction for Security Protocols},
  	volume =	{42},
  	year =	{2015},
}


@inproceedings{arapinis-csf10,
  author    = {Myrto Arapinis and
               Tom Chothia and
               Eike Ritter and
               Mark Ryan},
  title     = {Analysing Unlinkability and Anonymity Using the Applied
               Pi Calculus},
 publisher = {IEEE Computer Society Press},
  booktitle = {Proc.\  23rd  Computer Security Foundations
               Symposium (CSF'10)},
  year      = {2010},
  pages     = {107-121}
}


@article{DKR-jcs08,
       author =   {Delaune, St{\'e}phanie and Kremer, Steve and Ryan, Mark D.}, 
journal = {Journal of Computer Security}, 
   month = jul, 
   number = {4},
   volume = {17},
   pages = {435-487}, 
   publisher = {{IOS} Press}, 
       title =   {Verifying Privacy-type Properties of Electronic Voting Protocols}, 
       year =   {2008}, 
  }
@INPROCEEDINGS{BlanchetCADE05,
  AUTHOR = {Bruno Blanchet},
  TITLE = {An Automatic Security Protocol Verifier based on Resolution Theorem Proving (invited tutorial)},
  BOOKTITLE = {Proc.\ 20th International Conference on Automated Deduction (CADE-20)},
  YEAR = 2005,
  MONTH = {July},
 OPTnote = {Proverif},
}
@INPROCEEDINGS{sysdesc-CAV05,
  AUTHOR = {Armando, A. and Basin, D. and Boichut, Y. and Chevalier, Y. and
  Compagna, L. and Cuellar, J. and Hankes Drielsma, P. and H\'eam, P.-C. and
  Kouchnarenko, O. and Mantovani, J. and M\"odersheim, S. and von Oheimb, D.
  and Rusinowitch, M. and Santiago, J. and Turuani, M. and Vigan\`o, L. and
  Vigneron, L.},
  TITLE = {{The AVISPA Tool for the automated validation of internet security
  protocols and applications}},
  BOOKTITLE = {{Proc. 17th International Conference on Computer Aided Verification,
  CAV'2005}},
  PAGES = {281-285},
  PUBLISHER = {Springer},
  SERIES = {LNCS},
  VOLUME = {3576},
  YEAR = {2005}
}
@inproceedings{Cr2008Scyther,
  author	= {Cas Cremers},
  title		= {The {S}cyther {T}ool: Verification, Falsification, and Analysis of Security Protocols},
  year		= {2008},
  booktitle     = {Proc.\ 20th International Conference on Computer Aided Verification ({CAV}'08)},
  publisher     = {Springer},
  series        = {LNCS},
  pages         = {414--418},
  volume        = {5123/2008}
}

@inproceedings{tamarin,
  author    = {Benedikt Schmidt and
               Simon Meier and
               Cas Cremers and
               David Basin},
  title     = {Automated Analysis of {Diffie-Hellman} Protocols and Advanced
               Security Properties},
  pages     = {78-94},
  booktitle     = {Proc.\ 25th Computer Security Foundations Symposium ({CSF}'12)},
  publisher = {IEEE Computer Society Press},
  year      = {2012},
}


@Misc{ProVerif-sources,
  OPTkey = 	 {},
  author = 	 {Bruno Blanchet},
  title = 	 {ProVerif 1.91},
  howpublished = {http://prosecco.gforge.inria.fr/personal/bblanche/},
  OPTmonth = 	 {},
  OPTyear = 	 {},
  note = 	 {As downloaded on October 1st, 2015. See files in directory /examples/pitype/choice/},
  OPTannote = 	 {}
}

@inproceedings{backes08zero,
  author       = {Backes, Michael and Maffei, Matteo and Unruh, Dominique},
  title        = {Zero-Knowledge in the Applied Pi-calculus and Automated Verification of the Direct Anonymous Attestation Protocol},
  booktitle    = {Proc.\ 29th  Symposium on Security and Privacy ({S\&P}'08)},
  year         = {2008}
}

@inproceedings{CLC-CCS2008,
  author =        {Comon{-}Lundh, Hubert and Cortier, V{\'e}ronique},
  booktitle =     {{P}roc.\ 15th {ACM} {C}onference on
                   {C}omputer and {C}ommunications {S}ecurity
                   ({CCS}'08)},
  pages =         {109-118},
  publisher =     {ACM Press},
  title =         {Computational Soundness of Observational Equivalence},
  year =          {2008},
}

@InProceedings{chothia10,
  author = 	 {Tom Chothia and Vitaliy Smirnov},
  title = 	 {A Traceability Attack Against e-Passports},
  booktitle = {Proc. 14th International Conference on Financial Cryptography and Data Security (FC'10)},
  year = 	 {2010},
}
@InProceedings{blanchetTag03,
  author = 	 {Bruno Blanchet and Andreas Podelski},
  title = 	 {Verification of Cryptographic Protocols: Tagging Enforces Termination},
  booktitle = {Proc.\ International Conference on Foundations of Software Science and Computation Structures (FoSSaCS'03)},
pages = {136-152},
year = 	 {2003},
  volume = 	 {2620},
  series = 	 {LNCS},
}

@inproceedings{CCD-esorics15,
  	author =	{Chr{\'e}tien, R{\'e}my and Cortier, V{\'e}ronique and Delaune, St{\'e}phanie},
  	booktitle =	{{P}roc. 20th {E}uropean {S}ymposium on {R}esearch in {C}omputer {S}ecurity ({ESORICS}'15)},
  	publisher =	{Springer},
  	series =	{LNCS},
	title =	{Checking trace equivalence: How to get rid of nonces?},
  	year =	{2015},
}
@article{TCS2013-Vincent,
  author =        {Cheval, Vincent and Cortier, V{\'e}ronique and Delaune, St\'ephanie},
  journal =       {Theoretical Computer Science},
  publisher =     {Elsevier},
  title =         {Deciding equivalence-based properties using constraint solving},
  year =          {2013},
volume = {492},
pages = {1-39},

}
@inproceedings{CCK-esop12,
  author =	  {Chadha, Rohit and Ciob{\^a}c{\u{a}}, {\c{S}}tefan and Kremer, Steve},
  booktitle =     {{P}roc.\ 21th {E}uropean {S}ymposium on {P}rogramming ({ESOP}'12)},
  pages =         {108-127},
  publisher =     {Springer},
  series =        {LNCS},
  title =         {Automated verification of equivalence properties of
                  cryptographic protocols},
  volume =        {7211},
  year =          {2012},
  }


@Article{DS81,
  author = 	 {D. Denning and G. Sacco},
  title = 	 {Timestamps in key distributed protocols},
  journal = 	 {Communication of the ACM},
  year = 	 {1981},
  OPTkey = 	 {},
  volume = 	 {24},
  number = 	 {8},
  pages = 	 {533–535},
  }

@article{proverifphase,
  AUTHOR = {Bruno Blanchet and Mart{\'\i}n Abadi and C{\'e}dric Fournet},
  TITLE = {Automated Verification of Selected Equivalences for Security Protocols},
  JOURNAL = {Journal of Logic and Algebraic Programming},
  YEAR = 2008,
  VOLUME = 75,
  NUMBER = 1,
  PAGES = {3--51},
 }

@InProceedings{icalp2013,
  author = 	 {R\'emy Chr\'etien and V\'eronique Cortier and  St\'ephanie Delaune},
  title = 	 {From security protocols to pushdown automata},
  booktitle = {{P}roc.\ 40th {I}nternational
                   {C}olloquium on {A}utomata, {L}anguages and
                   {P}rogramming ({ICALP}'13)},
  pages = 	 {137-149},
  year = 	 {2013},
  OPTeditor = 	 {},
  volume = 	 {7966},
  series = 	 {LNCS},
  publisher = {Springer},
}

@inproceedings{pfitzmann2001anonymity,
  title={Anonymity, unobservability, and pseudonymity—a proposal for terminology},
  author={Pfitzmann, Andreas and K{\"o}hntopp, Marit},
  booktitle={Designing privacy enhancing technologies},
  pages={1--9},
  year={2001},
  organization={Springer}
}

@inproceedings{baudet2005deciding,
  title={Deciding security of protocols against off-line guessing attacks},
  author={Baudet, Mathieu},
  booktitle={Proc.\ 12th ACM conference on Computer and communications security ({CCS}'05)},
  pages={16--25},
  year={2005},
  organization={ACM}
}
@inproceedings{CCD-ijcar10,
   author = {Cheval, Vincent and Comon{-}Lundh, Hubert and Delaune, St{\'e}phanie},
   title = {Automating security analysis: symbolic equivalence of constraint systems},
   booktitle = {{P}roc.\  5th {I}nternational {J}oint {C}onference on {A}utomated {R}easoning ({IJCAR}'10)},
   year = {2010},
   volume = {6173},
   pages = {412-426},
   series = {LNAI},
   publisher = {Springer-Verlag},
  }

@inproceedings{CCD-ccs11,
   author = {Cheval, Vincent and Comon{-}Lundh, Hubert and Delaune, St{\'e}phanie},
   title = {Trace Equivalence Decision: Negative Tests and Non-determinism},
   booktitle = {{P}roc.\  18th {ACM} {C}onference on {C}omputer and {C}ommunications {S}ecurity ({CCS}'11)},
   year = {2011},
   pages = {321-330},
   publisher = {ACM Press},
}

@inproceedings{Cheval-tacas14,
   author = {Cheval, Vincent},
   title = {APTE: an Algorithm for Proving Trace Equivalence},
   booktitle = {{P}roc.\ 20th {I}nternational {C}onference on {T}ools and {A}lgorithms for the {C}onstruction and {A}nalysis of {S}ystems ({TACAS}'14)},
   year = {2014},
   volume = {8413},
   pages = {587-592},
   series = {LNCS},
   }


@inproceedings{CCP-cav13,
  author = {Cheval, Vincent and Cortier, V{\'e}ronique and Plet, Antoine},
  title = {Lengths may break privacy -- or how to check for equivalences with length},
  booktitle = {Proc.\ 25th International Conference on Computer Aided Verification (CAV'13)},
  year = {2013},
  volume = {8044},
  pages = {708-723},
  series = {LNCS},
  publisher = {Springer Berlin Heidelberg},
  }

@inproceedings{cheval2015timing,
  title={Timing attacks in security protocols: symbolic framework and proof techniques},
  author={Cheval, Vincent and Cortier, V{\'e}ronique},
  booktitle={Proc. 4th  Conference on Principles of Security and Trust ({POST}'15)},
  pages={280--299},
  year={2015},
  publisher={Springer}
}

@inproceedings{tiu2010automating,
  title={Automating open bisimulation checking for the spi calculus},
  author={Tiu, Alwen and Dawson, Jeremy},
  booktitle={Proc.\ 23rd Computer Security Foundations Symposium (CSF'10)},
  pages={307--321},
  year={2010},
  organization={IEEE Computer Society Press}
}

@inproceedings{tiu2007trace,
  title={A trace based bisimulation for the spi calculus},
  author={Tiu, Alwen},
  booktitle={Programming Languages and Systems},
  pages={367--382},
  year={2007},
  publisher={Springer}
}

@ARTICLE{BlanchetAbadiFournetJLAP07,
  AUTHOR = {Bruno Blanchet and Mart{\'\i}n Abadi and C{\'e}dric Fournet},
    TITLE = {Automated Verification of Selected Equivalences for Security Protocols},
      JOURNAL = {Journal of Logic and Algebraic Programming},
        YEAR = 2008,
	  VOLUME = 75,
	    NUMBER = 1,
	      PAGES = {3--51},
	       	}




@INPROCEEDINGS{BlanchetAbadiFournetLICS05,
  AUTHOR = {Bruno Blanchet and Mart{\'\i}n Abadi and C{\'e}dric Fournet},
    TITLE = {Automated {V}erification of {S}elected {E}quivalences for {S}ecurity {P}rotocols},
      BOOKTITLE = {Proc.\ 20th Symposium on Logic in Computer Science (LICS'05)},
        PAGES = {331--340},
	  YEAR = 2005,
	        PUBLISHER = {IEEE Computer Society Press}
		}



@INPROCEEDINGS{ChevalBlanchetPOST13,
  AUTHOR = {Vincent Cheval and Bruno Blanchet},
    TITLE = {Proving More Observational Equivalences with {P}ro{V}erif},
      BOOKTITLE = {Proc.\ 2nd Conference on Principles of Security and Trust (POST'13)},
        PAGES = {226--246},
	  YEAR = 2013,
	      VOLUME = 7796,
	        SERIES = {LNCS},
		      PUBLISHER = {Springer}
		      }

@inproceedings{santiago2014formal,
  title={A formal definition of protocol indistinguishability and its verification using {Maude-NPA}},
    author={Santiago, Sonia and Escobar, Santiago and Meadows, Catherine and Meseguer, Jos{\'e}},
      booktitle={Security and Trust Management},
        pages={162--177},
	  year={2014},
	    publisher={Springer}
	    }


@inproceedings{escobar2010folding,
  title={Folding variant narrowing and optimal variant termination},
    author={Escobar, Santiago and Sasse, Ralf and Meseguer, Jos{\'e}},
      booktitle={Rewriting Logic and Its Applications},
        pages={52--68},
	  year={2010},
	    publisher={Springer}
	    }

@inproceedings{basin2015automated,
  title={Automated symbolic proofs of observational equivalence},
    author={Basin, David and Dreier, Jannik and Sasse, Ralf},
      booktitle={Proc.\ 22nd  Conference on Computer and Communications Security (CCS'15)},
        pages={1144--1155},
	  year={2015},
	    organization={ACM}
	    }


@inproceedings{meier2013tamarin,
  title={The tamarin prover for the symbolic analysis of security protocols},
    author={Meier, Simon and Schmidt, Benedikt and Cremers, Cas and Basin, David},
      booktitle={Proc. International Conference on Computer Aided Verification (CAV'13)},
        pages={696--701},
	  year={2013},
	    organization={Springer}
	    }

@inproceedings{cortier2011attacking,
  title={Attacking and fixing Helios: An analysis of ballot secrecy},
    author={Cortier, V{\'e}ronique and Smyth, Brendan},
      booktitle={Proc. 24th Computer Security Foundations Symposium (CSF'11)},
        pages={297--311},
	  year={2011},
	    organization={IEEE Computer Society Press}
	    }


@inproceedings{cortier2012formal,
  title={A formal analysis of the Norwegian E-voting protocol},
    author={Cortier, V{\'e}ronique and Wiedling, Cyrille},
      booktitle={Proc. 2nd Conference on Principles of Security and Trust},
        pages={109--128},
	  year={2012},
	    publisher={Springer}
	    }

@inproceedings{arapinis2012new,
  title={New privacy issues in mobile telephony: fix and verification},
    author={Arapinis, Myrto and Mancini, Loretta and Ritter, Eike and Ryan, Mark and Golde, Nico and Redon, Kevin and Borgaonkar, Ravishankar},
      booktitle={Proc. ACM conference on Computer and Communications Security (CCS'12)},
        pages={205--216},
	  year={2012},
	    organization={ACM}
	    }

@inproceedings{arapinis2014privacy,
  title={Privacy through pseudonymity in mobile telephony systems},
    author={Arapinis, Myrto and Mancini, Loretta Ilaria and Ritter, Eike and Ryan, Mark},
      booktitle={Proc. Network and Distributed System Security Symposium (NDSS'14)},
        year={2014}
	}


@inproceedings{bruso2010formal,
  title={Formal verification of privacy for {RFID} systems},
    author={Brus{\'o}, Mayla and Chatzikokolakis, Konstantinos and Den Hartog, Jerry},
      booktitle={Proc.\ 23rd Computer Security Foundations Symposium (CSF'10)},
        pages={75--88},
	  year={2010},
	    organization={IEEE Computer Society Press}
	    }


@inproceedings{cortier2015type,
  title={Type-Based Verification of Electronic Voting Protocols},
    author={Cortier, V{\'e}ronique and Eigner, Fabienne and Kremer, Steve and Maffei, Matteo and Wiedling, Cyrille},
      booktitle={Proc.\ 4th Conference on Principles of Security and Trust (POST'15)},
        pages={303--323},
	  year={2015},
	    publisher={Springer}
	    }

@inproceedings{barthe2014probabilistic,
  title={Probabilistic relational verification for cryptographic implementations},
    author={Barthe, Gilles and Fournet, C{\'e}dric and Gr{\'e}goire, Benjamin and Strub, Pierre-Yves and Swamy, Nikhil and Zanella-B{\'e}guelin, Santiago},
      booktitle={Proc.\ 41st Symposium on Principles of Programming Languages ({POPL}'14)},
        volume={49},
	    pages={193-206},
	      year={2014},
	        organization={ACM}
		}
@article{cheval2013deciding,
  title={Deciding equivalence-based properties using constraint solving},
    author={Cheval, Vincent and Cortier, V{\'e}ronique and Delaune, St{\'e}phanie},
      journal={Theoretical Computer Science},
        volume={492},
	  pages={1--39},
	    year={2013},
	      publisher={Elsevier}
	      }
	      


@inproceedings{chadha2012automated,
  title={Automated verification of equivalence properties of cryptographic protocols},
    author={Chadha, Rohit and Ciob{\^a}c{\u{a}}, {\c{S}}tefan and Kremer, Steve},
      booktitle={Proc. European Symposium on Programming (ESOP'12)},
        pages={108--127},
	  year={2012},
	    publisher={Springer}
	    }


@inproceedings{chretien2013security,
  title={From security protocols to pushdown automata},
    author={Chr{\'e}tien, R{\'e}my and Cortier, V{\'e}ronique and Delaune, St{\'e}phanie},
      booktitle={Automata, Languages, and Programming},
        pages={137--149},
	  year={2013},
	    publisher={Springer}
	    }


@article{huttel2003deciding,
  title={Deciding framed bisimilarity},
    author={H{\"u}ttel, Hans},
      journal={Electronic Notes in Theoretical Computer Science},
        volume={68},
	  number={6},
	    pages={1--18},
	      year={2003},
	        publisher={Elsevier}
		}

@inproceedings{comon2005finite,
  title={The finite variant property: How to get rid of some algebraic properties},
    author={Comon-Lundh, Hubert and Delaune, St{\'e}phanie},
      booktitle={Proc. International Conference on Rewriting Techniques and Applications (RTA'05)},
        pages={294--307},
	  year={2005},
	    publisher={Springer}
	    }


@inproceedings{baelde2014reduced,
  title={A reduced semantics for deciding trace equivalence using constraint systems},
    author={Baelde, David and Delaune, St{\'e}phanie and Hirschi, Lucca},
      booktitle={Proc.\ 3rd Conference on Principles of Security and Trust (POST'14)},
        pages={1--21},
	  year={2014},
	    publisher={Springer}
	    }
@inproceedings{bana2014computationally,
  title={A computationally complete symbolic attacker for equivalence properties},
    author={Bana, Gergei and Comon-Lundh, Hubert},
      booktitle={Proc.\  21st Conference on Computer and Communications Security (CCS'14))},
        pages={609--620},
	  year={2014},
	    organization={ACM}
	    }

@inproceedings{blanchet2004automatic,
  title={Automatic proof of strong secrecy for security protocols},
    author={Blanchet, Bruno},
      booktitle={Proc.\ . 2004 Symposium on Security and Privacy},
        pages={86--100},
	  year={2004},
	    organization={IEEE Computer Society Press}
	    }

@inproceedings{abadi1997secrecy,
  title={Secrecy by typing in security protocols},
    author={Abadi, Martin},
      booktitle={Theoretical Aspects of Computer Software},
        pages={611--638},
	  year={1997},
	    organization={Springer}
	    }

@inproceedings{abadi1997calculus,
  title={A calculus for cryptographic protocols: The spi calculus},
    author={Abadi, Mart{\'\i}n and Gordon, Andrew D},
      booktitle={Proc.\ of the 4th ACM conference on Computer and communications security},
        pages={36--47},
	  year={1997},
	    organization={ACM}
	    }


@article{AbadiG98,
  author    = {Mart{\'{\i}}n Abadi and
               Andrew D. Gordon},
  title     = {A Bisimulation Method for Cryptographic Protocols},
  journal   = {Nord. J. Comput.},
  volume    = {5},
  number    = {4},
  pages     = {267},
  year      = {1998},
  timestamp = {Wed, 14 Jan 2004 15:33:49 +0100},
  OPTbiburl    = {http://dblp.uni-trier.de/rec/bib/journals/njc/AbadiG98},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{psi-calculus,
  author    = {Jesper Bengtson and
               Magnus Johansson and
               Joachim Parrow and
               Bj{\"{o}}rn Victor},
  title     = {Psi-calculi: a framework for mobile processes with nominal data and
               logic},
  journal   = {Logical Methods in Computer Science},
  volume    = {7},
  number    = {1},
  year      = {2011},
  }

@article{DKR-jcs09,
   author = {Delaune, St{\'e}phanie and Kremer, Steve and Ryan, Mark D.}, 
   journal = {Journal of Computer Security}, 
   month = mar, 
   number = {2}, 
   pages = {317-377}, 
   publisher = {{IOS} Press}, 
   title = {Symbolic bisimulation for the applied pi~calculus}, 
   volume = {18}, 
   year = {2010}, 
}

@article{Borgstrom09,
  author    = {Johannes Borgstr{\"{o}}m},
  title     = {A Complete Symbolic Bisimilarity for an Extended Spi Calculus},
  journal   = {Electr. Notes Theor. Comput. Sci.},
  volume    = {242},
  number    = {3},
  pages     = {3--20},
  year      = {2009},
 }

@article{BorgstromGRV15,
  author    = {Johannes Borgstr{\"{o}}m and
               Ramunas Gutkovas and
               Ioana Rodhe and
               Bj{\"{o}}rn Victor},
  title     = {The Psi-Calculi Workbench: {A} Generic Tool for Applied Process Calculi},
  journal   = {{ACM} Trans. Embedded Comput. Syst.},
  volume    = {14},
  number    = {1},
  pages     = {9:1--9:25},
  year      = {2015},
 }

@inproceedings{ArapinisBR12,
  author    = {Myrto Arapinis and
               Sergiu Bursuc and
               Mark Dermot Ryan},
  title     = {Reduction of Equational Theories for Verification of Trace Equivalence:
               Re-encryption, Associativity and Commutativity},
  booktitle = {Proc.\ 1st International Conference on Principles of Security and Trust ({POST}'12)},
  pages     = {169--188},
  year      = {2012},
  series    = {LNCS},
  volume    = {7215},
  publisher = {Springer},
 }

@inproceedings{DBLP:conf/sp/Blanchet06,
  author    = {Bruno Blanchet},
    title     = {A Computationally Sound Mechanized Prover for Security Protocols},
      booktitle = {Proc.\ Symposium on Security and Privacy (S{\&}P'06)},
       pages     = {140--154},
         year      = {2006},
	 publisher = {IEEE Computer Society Press},
	   biburl    = {http://dblp.uni-trier.de/rec/bib/conf/sp/Blanchet06},
	     bibsource = {dblp computer science bibliography, http://dblp.org}
     }

@inproceedings{DBLP:conf/ifipTCS/AbadiR00,
  author    = {Mart{\'{\i}}n Abadi and
                 Phillip Rogaway},
   title     = {Reconciling Two Views of Cryptography (The Computational Soundness
                 of Formal Encryption)},
    booktitle = {Proc.\ International Conference on Theoretical Computer Science},
    pages     = {3-22},
    year      = {2000},
   }

@article{cortier2011survey,
  title={A survey of symbolic methods in computational analysis of cryptographic systems},
    author={Cortier, V{\'e}ronique and Kremer, Steve and Warinschi, Bogdan},
      journal={Journal of Automated Reasoning},
        volume={46},
	  number={3-4},
	    pages={225--259},
	      year={2011},
	        publisher={Springer-Verlag New York, Inc.}
		}


@inproceedings{bana2012towards,
  title={Towards unconditional soundness: Computationally complete symbolic attacker},
    author={Bana, Gergei and Comon-Lundh, Hubert},
      booktitle={Proc.\ 1st International Conference on Principles of Security and Trust (POST'12)},
        pages={189--208},
	  year={2012},
	    publisher={Springer}
	    }


@inproceedings{arapinis2009untraceability,
  title={Untraceability in the applied pi-calculus},
    author={Arapinis, Myrto and Chothia, Tom and Ritter, Eike and Ryan, Mark},
      booktitle={Proc.\ International Conference for Internet Technology and Secured Transactions ({ICITST},09)},
        pages={1--6},
	  year={2009},
	    organization={IEEE Computer Society Press}
	    }

@inproceedings{bruso2013linking,
  title={Linking unlinkability},
    author={Brus{\'o}, Mayla and Chatzikokolakis, Konstantinos and Etalle, Sandro and Den Hartog, Jerry},
      booktitle={Trustworthy Global Computing},
        pages={129--144},
	  year={2013},
	    publisher={Springer}
	    }


@inproceedings{van2008untraceability,
  title={Untraceability of {RFID} protocols},
    author={Van Deursen, Ton and Mauw, Sjouke and Radomirovi{\'c}, Sa{\v{s}}a},
      booktitle={Information Security Theory and Practices. Smart Devices, Convergence and Next Generation Networks},
        pages={1--15},
	  year={2008},
	    publisher={Springer}
	    }

@inproceedings{van2009algebraic,
  title={Algebraic attacks on {RFID} protocols},
    author={van Deursen, Ton and Radomirovi{\'c}, Sa{\v{s}}a},
      booktitle={Information Security Theory and Practice. Smart Devices, Pervasive Systems, and Ubiquitous Networks},
        pages={38--51},
	  year={2009},
	    publisher={Springer}
	    }

@inproceedings{schneider1996csp,
  title={{CSP} and anonymity},
    author={Schneider, Steve and Sidiropoulos, Abraham},
      booktitle={Proc.\ International Conference on Computer Security (ESORICS'96)},
        pages={198--218},
	  year={1996},
	    organization={Springer}
	    }

@inproceedings{garcia2005provable,
  title={Provable anonymity},
    author={Garcia, Flavio D and Hasuo, Ichiro and Pieters, Wolter and Van Rossum, Peter},
      booktitle={Proc.\  of the 2005 ACM workshop on Formal methods in security engineering},
        pages={63--72},
	  year={2005},
	    organization={ACM}
	    }

@inproceedings{chothia2006analysing,
  title={Analysing the MUTE anonymous file-sharing system using the pi-calculus},
    author={Chothia, Tom},
      booktitle={Formal Techniques for Networked and Distributed Systems-FORTE 2006},
        pages={115--130},
	  year={2006},
	    publisher={Springer}
	    }
								}
@inproceedings{HBD-sp16,
  author       = {Hirschi, Lucca and Baelde, David and Delaune, St{\'e}phanie},
  title        = {A~method for verifying privacy-type properties: the~unbounded case},
  booktitle    = {Proc.\ 37th  Symposium on Security and Privacy ({S\&P}'16)},
  year         = {2016},
  note = "To appear"
 }
@inproceedings{2016-verifying-observational-equivalence,
       author = "Bruno Blanchet and Ben Smyth",
       title = "Automated reasoning for equivalences in the applied pi calculus with barriers",
       year = "2016", 
       booktitle = {{P}roc.\  29th {C}omputer {S}ecurity {F}oundations {S}ymposium ({CSF}'16)},
       note = "To appear",
    }

@inproceedings{arapinis2016three,
   title={When are three voters enough for privacy properties?},
   author={Arapinis, Myrto and Cortier, V{\'e}ronique and Kremer, Steve},
   booktitle={European Symposium on Research in Computer Security (ESORICS'16)},
   pages={241--260},
   year={2016},
   organization={Springer}
   }
	    
